Recurrence of the Uniform Infinite Half-Plane Map via duality of resistances

We study the simple random walk on the Uniform Infinite Half-Plane Map, which is the local limit of critical Boltzmann planar maps with a large and simple boundary. We prove that the simple random walk is recurrent, and that the resistance between the root and the boundary of the hull of radius $r$ is at least of order $\log r$. This resistance bound is expected to be sharp, and is better than those following from previous proofs of recurrence for non bounded-degree planar maps models. Our main tools are the self-duality of uniform planar maps, a classical lemma about duality of resistances and some peeling estimates. The proof shares some ideas with Russo--Seymour--Welsh theory in percolation.

==> mes-commandes.tex <==


% Raccourcis génériques souvent employés
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
%\newcommand{\ud}{\text{d}}
% Les doubles barres
\newcommand{\1}{\mathds{1}}
\DeclareMathOperator{\id}{id}
\newcommand{\eqdistr}{\overset{\operatorname{(d)}}{=}}
\newcommand{\eqdef}{\overset{\text{def}}{=}}
\newcommand{\cste}{{\operatorname{const} \cdot}}
\newcommand{\card}[1]{\left| #1 \right|}
\newcommand{\floor}[1]{{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{{\left\lceil #1 \right\rceil}}
\newcommand{\usim}[2]{\underset{#1 \to #2}{\sim}}
\newcommand{\usiminc}[2]{\underset{#1 \nearrow #2}{\sim}}
\newcommand{\ulim}[2]{\underset{#1 \to #2}{\longrightarrow}}
\newcommand{\uliminc}[2]{\underset{#1 \nearrow #2}{\longrightarrow}}
\newcommand{\ulimd}[2]{\overset{\textrm{(d)}}{\ulim{#1}{#2}}}
\newcommand{\ulimincd}[2]{\overset{\textrm{(d)}}{\uliminc{#1}{#2}}}
\newcommand{\ulimas}[2]{\overset{\textrm{\as}}{\ulim{#1}{#2}}}
\newcommand{\pfrac}[2]{{\left(\frac{#1}{#2}\right)}}
\newcommand{\too}{\longrightarrow}
\newcommand{\figref}[1]{Figure \ref{#1}}


% Abréviations usuelles
\newcommand{\ps}{\text{p.s.}\xspace}
\newcommand{\as}{\text{a.s.}\xspace}
\newcommand{\whp}{\text{w.h.p.}\xspace}
\newcommand{\wrt}{\text{w.r.t.}\xspace}
\newcommand{\iid}{\text{i.i.d.}\xspace}
\newcommand{\resp}{\text{resp.}\xspace}
\newcommand{\ie}{\textit{i.e.}\xspace}



% Raccourcis plus spécifiques
\DeclareMathOperator{\Krikun}{Krikun}
\newcommand{\Inn}{\operatorname{Inn}}
\newcommand{\fpp}{\text{fpp}}
\DeclareMathOperator{\skel}{Skel}
\DeclareMathOperator{\slots}{Slots}
\DeclareMathOperator{\core}{Core}
\newcommand{\dgr}{\mathrm{d}_{\mathrm{gr}}}
\newcommand{\dmap}{\mathrm{d}_{\mathrm{map}}}
\newcommand{\dTutte}{\mathrm{d}_{\mathrm{Tutte}}}
\newcommand{\ddual}{\mathrm{d}_{\mathrm{fpp}}^\dagger}
\newcommand{\dfpp}{\mathrm{d}_{\mathrm{fpp}}}
\newcommand{\Htr}{\HH^\text{tr}}




% Commandes de texte
\newcommand{\uipq}{\text{uniform infinite planar quadrangulation}\xspace}
\newcommand{\Uipq}{\text{Uniform infinite planar quadrangulation}\xspace}
%\newcommand{\UIPQ}{\textsc{uipq}\xspace}
\newcommand{\uhpq}{\text{upper half plane quadrangulation}\xspace}
\newcommand{\Uhpq}{\text{Upper half plane quadrangulation}\xspace}
\newcommand{\UHPQ}{\textsc{uhpq}\xspace}
\newcommand{\uhpm}{\text{uniform half plane map}\xspace}
\newcommand{\Uhpm}{\text{Uniform half plane map}\xspace}
\newcommand{\UHPM}{\textsc{uhpm}\xspace}
%\newcommand{\UIHPQ}{\textsc{uihpq}\xspace}
\newcommand{\lhpq}{\text{lower half plane quadrangulation}\xspace}
\newcommand{\Lhpq}{\text{Lower half plane quadrangulation}\xspace}
\newcommand{\LHPQ}{\textsc{lhpq}\xspace}
\newcommand{\QPPM}{\textsc{qppm}\xspace}
\DeclareMathOperator{\Bin}{Bin}





% Package color
%OK
% red, blue, green, white, black, cyan, magenta, yellow
%NON OK
% purple, olive, teal, violet, brown, darkgray, gray, lightgray, lime, orange, pink
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\newcommand{\correct}{\textcolor{red}}
\newcommand{\anticipate}{\textcolor{blue}}
\newcommand{\generally}{\textcolor{green}}
\newcommand{\redac}{\textcolor{magenta}}
\newcommand{\illustration}{\begin{center} \generally{\textsc{Illustration requise.}}\end{center}}





%%%%%%%%%%%%%%%%% BUDZ %%%%%%%%%%%%%%%%%%

\newcommand{\Reff}{R_\mathrm{eff}}
\newcommand{\ttime}{\tau_{\mathrm{time}}}
\newcommand{\twalk}{\tau_{\mathrm{walk}}}
\newcommand{\tjump}{\tau_{\mathrm{jump}}}


==> mes-lettres.tex <==

% Raccourcis : mise en forme. Utiliser plutôt \operatorname ?
% DROIT
\newcommand\ov{\overline}
\newcommand\un{\underline}
\newcommand\wt{\widetilde}
\newcommand\wh{\widehat}




% GRAS			proposition : \b<lettre>, la casse passant à la commande.
\newcommand\ba{\textbf{a}}
\newcommand\bb{\textbf{b}}
\newcommand\bc{\textbf{c}}
\newcommand\bd{\textbf{d}}
\newcommand\be{\textbf{e}}
\renewcommand\bf{\textbf{f}}		% gras (préférer \textbf ou \mathbf, plus récents)
\newcommand\bg{\textbf{g}}
\newcommand\bh{\textbf{h}}
\newcommand\bi{\textbf{i}}
\newcommand\bj{\textbf{j}}
\newcommand\bk{\textbf{k}}
\newcommand\bl{\textbf{l}}
\newcommand\bm{\textbf{m}}
\newcommand\bn{\textbf{n}}
\newcommand\bo{\textbf{o}}
\newcommand\bp{\textbf{p}}
\newcommand\bq{\textbf{q}}
\newcommand\br{\textbf{r}}
\newcommand\bs{\textbf{s}}
\newcommand\bt{\textbf{t}}
\newcommand\bu{\textbf{u}}
\newcommand\bv{\textbf{v}}
\newcommand\bw{\textbf{w}}
\newcommand\bx{\textbf{x}}
\newcommand\by{\textbf{y}}
\newcommand\bz{\textbf{z}}

\newcommand\bA{\textbf{A}}
\newcommand\bB{\textbf{B}}
\newcommand\bC{\textbf{C}}
\newcommand\bD{\textbf{D}}
\newcommand\bE{\textbf{E}}
\newcommand\bF{\textbf{F}}
\newcommand\bG{\textbf{G}}
\newcommand\bH{\textbf{H}}
\newcommand\bI{\textbf{I}}
\newcommand\bJ{\textbf{J}}
\newcommand\bK{\textbf{K}}
\newcommand\bL{\textbf{L}}
\newcommand\bM{\textbf{M}}
\newcommand\bN{\textbf{N}}
\newcommand\bO{\textbf{O}}
\newcommand\bP{\textbf{P}}
\newcommand\bQ{\textbf{Q}}
\newcommand\bR{\textbf{R}}
\newcommand\bS{\textbf{S}}
\newcommand\bT{\textbf{T}}
\newcommand\bU{\textbf{U}}
\newcommand\bV{\textbf{V}}
\newcommand\bW{\textbf{W}}
\newcommand\bX{\textbf{X}}
\newcommand\bY{\textbf{Y}}
\newcommand\bZ{\textbf{Z}}




% Mathrm			proposition : \u<lettre>, la casse passant à la commande.
\newcommand\ua{\textrm{a}}
\newcommand\ub{\textrm{b}}
\newcommand\uc{\textrm{c}}
\newcommand\ud{\textrm{d}}
\newcommand\ue{\textrm{e}}
\newcommand\uf{\textrm{f}}
\newcommand\ug{\textrm{g}}
\newcommand\uh{\textrm{h}}
\newcommand\ui{\textrm{i}}
\newcommand\uj{\textrm{j}}
\newcommand\uk{\textrm{k}}
\newcommand\ul{\textrm{l}}
\newcommand\um{\textrm{m}}
%\newcommand\un{\textrm{n}}
\newcommand\uo{\textrm{o}}
\newcommand\up{\textrm{p}}
\newcommand\uq{\textrm{q}}
\newcommand\ur{\textrm{r}}
\newcommand\us{\textrm{s}}
\newcommand\ut{\textrm{t}}
\newcommand\uu{\textrm{u}}
\newcommand\uv{\textrm{v}}
\newcommand\uw{\textrm{w}}
\newcommand\ux{\textrm{x}}
\newcommand\uy{\textrm{y}}
\newcommand\uz{\textrm{z}}



% FRAK
\newcommand\ka{\mathfrak{a}}
\newcommand\kb{\mathfrak{b}}
\newcommand\kc{\mathfrak{c}}
\newcommand\kd{\mathfrak{d}}
\newcommand\ke{\mathfrak{e}}
\newcommand\kf{\mathfrak{f}}		
\newcommand\kg{\mathfrak{g}}
\newcommand\kh{\mathfrak{h}}
\newcommand\ki{\mathfrak{i}}
\newcommand\kj{\mathfrak{j}}
\newcommand\kk{\mathfrak{k}}
\newcommand\kl{\mathfrak{l}}
\newcommand\km{\mathfrak{m}}
\newcommand\kn{\mathfrak{n}}
\newcommand\ko{\mathfrak{o}}
\newcommand\kp{\mathfrak{p}}
\newcommand\kq{\mathfrak{q}}
\newcommand\kr{\mathfrak{r}}
\newcommand\ks{\mathfrak{s}}
\newcommand\kt{\mathfrak{t}}
\newcommand\ku{\mathfrak{u}}
\newcommand\kv{\mathfrak{v}}
\newcommand\kw{\mathfrak{w}}
\newcommand\kx{\mathfrak{x}}
\newcommand\ky{\mathfrak{y}}
\newcommand\kz{\mathfrak{z}}

\newcommand\kA{\mathfrak{A}}
\newcommand\kB{\mathfrak{B}}
\newcommand\kC{\mathfrak{C}}
\newcommand\kD{\mathfrak{D}}
\newcommand\kE{\mathfrak{E}}
\newcommand\kF{\mathfrak{F}}
\newcommand\kG{\mathfrak{G}}
\newcommand\kH{\mathfrak{H}}
\newcommand\kI{\mathfrak{I}}
\newcommand\kJ{\mathfrak{J}}
\newcommand\kK{\mathfrak{K}}
\newcommand\kL{\mathfrak{L}}
\newcommand\kM{\mathfrak{M}}
\newcommand\kN{\mathfrak{N}}
\newcommand\kO{\mathfrak{O}}
\newcommand\kP{\mathfrak{P}}
\newcommand\kQ{\mathfrak{Q}}
\newcommand\kR{\mathfrak{R}}
\newcommand\kS{\mathfrak{S}}
\newcommand\kT{\mathfrak{T}}
\newcommand\kU{\mathfrak{U}}
\newcommand\kV{\mathfrak{V}}
\newcommand\kW{\mathfrak{W}}
\newcommand\kX{\mathfrak{X}}
\newcommand\kY{\mathfrak{Y}}
\newcommand\kZ{\mathfrak{Z}}



% MATHBB		proposition : \<majuscule> ou \<double majuscule>
\newcommand\A{\mathbb{A}}
\newcommand\B{\mathbb{B}}
\newcommand\C{\mathbb{C}}
\newcommand\D{\mathbb{D}}
\newcommand\E{\mathbb{E}}
\newcommand\F{\mathbb{F}}
\newcommand\G{\mathbb{G}}
\renewcommand\H{\mathbb{H}}		% Umlaut
\newcommand\I{\mathbb{I}}
\newcommand\J{\mathbb{J}}
\newcommand\K{\mathbb{K}}
\renewcommand\L{\mathbb{L}}		% Ł barré majuscule polonais
\newcommand\M{\mathbb{M}}
\newcommand\N{\mathbb{N}}
\renewcommand\O{\mathbb{O}}		% Ø scandinave
\renewcommand\P{\mathbb{P}}		% ¶ paragraphe
\newcommand\Q{\mathbb{Q}}
\newcommand\R{\mathbb{R}}
\renewcommand\S{\mathbb{S}}		% § paragraphe
\newcommand\T{\mathbb{T}}
\newcommand\U{\mathbb{U}}
\newcommand\V{\mathbb{V}}
\newcommand\W{\mathbb{W}}
\newcommand\X{\mathbb{X}}
\newcommand\Y{\mathbb{Y}}
\newcommand\Z{\mathbb{Z}}



% MATHCAL		proposition : SOIT \<minuscule> mais beaucoup de conflits, SOIT \<double minuscule>, SOIT \<double majuscule>
%\newcommand\aa{\mathcal{A}}		% a accentué avec un rond scandinave
%\newcommand\bb{\mathcal{B}}
%\newcommand\cc{\mathcal{C}}
%\newcommand\dd{\mathcal{D}}
%\newcommand\ee{\mathcal{E}}
%\newcommand\ff{\mathcal{F}}
%\newcommand\gg{\mathcal{G}}		% double > (difficilement évitable)
%\newcommand\hh{\mathcal{H}}
%\newcommand\ii{\mathcal{I}}
%\newcommand\jj{\mathcal{J}}
%\newcommand\kk{\mathcal{K}}
%\newcommand\ll{\mathcal{L}}		%  double < (difficilement évitable)
%\newcommand\mm{\mathcal{M}}
%\newcommand\nn{\mathcal{N}}
%\newcommand\oo{\mathcal{O}}
%\newcommand\pp{\mathcal{P}}
%\newcommand\qq{\mathcal{Q}}		%  \mathrm{q} au-dessus
%\newcommand\rr{\mathcal{R}}
%\newcommand\ss{\mathcal{S}}		% Eszett allemand
%\newcommand\tt{\mathcal{T}}		% verbatim
%\newcommand\uu{\mathcal{U}}
%\newcommand\vv{\mathcal{V}}
%\newcommand\ww{\mathcal{W}}
%\newcommand\xx{\mathcal{X}}
%\newcommand\yy{\mathcal{Y}}
%\newcommand\zz{\mathcal{Z}}


% Avec le package rsfso : plus arrondi et joli.
% On peut utiliser \mathscr, qui donnera la même chose en plus italique.

\renewcommand\AA{\mathcal{A}}		% A scandinave accentué avec un rond
\newcommand\BB{\mathcal{B}}
\newcommand\CC{\mathcal{C}}
\newcommand\DD{\mathcal{D}}
\newcommand\EE{\mathcal{E}}
\newcommand\FF{\mathcal{F}}
\newcommand\GG{\mathcal{G}}
\newcommand\HH{\mathcal{H}}
\newcommand\II{\mathcal{I}}
\newcommand\JJ{\mathcal{J}}
\newcommand\KK{\mathcal{K}}
\newcommand\LL{\mathcal{L}}
\newcommand\MM{\mathcal{M}}
\newcommand\NN{\mathcal{N}}
\newcommand\OO{\mathcal{O}}
\newcommand\PP{\mathcal{P}}
\newcommand\QQ{\mathcal{Q}}
\newcommand\RR{\mathcal{R}}
\renewcommand\SS{\mathcal{S}}		% Eszett majuscule, affiché comme "SS".
\newcommand\TT{\mathcal{T}}
\newcommand\UU{\mathcal{U}}
\newcommand\VV{\mathcal{V}}
\newcommand\WW{\mathcal{W}}
\newcommand\XX{\mathcal{X}}
\newcommand\YY{\mathcal{Y}}
\newcommand\ZZ{\mathcal{Z}}



% TILDE - Pas besoin avec \wt
%\newcommand{\tA}{\widetilde{A}}
%\newcommand{\tB}{\widetilde{B}}
%\newcommand{\tC}{\widetilde{C}}
%\newcommand{\tD}{\widetilde{D}}
%\newcommand{\tE}{\widetilde{E}}
%\newcommand{\tF}{\widetilde{F}}
%\newcommand{\tG}{\widetilde{G}}
%\newcommand{\tH}{\widetilde{H}}
%\newcommand{\tI}{\widetilde{I}}
%\newcommand{\tJ}{\widetilde{J}}
%\newcommand{\tK}{\widetilde{K}}
%\newcommand{\tL}{\widetilde{L}}
%\newcommand{\tM}{\widetilde{M}}
%\newcommand{\tN}{\widetilde{N}}
%\newcommand{\tO}{\widetilde{O}}
%\newcommand{\tP}{\widetilde{P}}
%\newcommand{\tQ}{\widetilde{Q}}
%\newcommand{\tR}{\widetilde{R}}
%\newcommand{\tS}{\widetilde{S}}
%\newcommand{\tT}{\widetilde{T}}
%\newcommand{\tU}{\widetilde{U}}
%\newcommand{\tV}{\widetilde{V}}
%\newcommand{\tW}{\widetilde{W}}
%\newcommand{\tX}{\widetilde{X}}
%\newcommand{\tY}{\widetilde{Y}}
%\newcommand{\tZ}{\widetilde{Z}}


% TILDE PLUS CAL - Pas besoin avec \wt
%\newcommand{\tAA}{\widetilde{\mathcal{A}}}
%\newcommand{\tBB}{\widetilde{\mathcal{B}}}
%\newcommand{\tCC}{\widetilde{\mathcal{C}}}
%\newcommand{\tDD}{\widetilde{\mathcal{D}}}
%\newcommand{\tEE}{\widetilde{\mathcal{E}}}
%\newcommand{\tFF}{\widetilde{\mathcal{F}}}
%\newcommand{\tGG}{\widetilde{\mathcal{G}}}
%\newcommand{\tHH}{\widetilde{\mathcal{H}}}
%\newcommand{\tII}{\widetilde{\mathcal{I}}}
%\newcommand{\tJJ}{\widetilde{\mathcal{J}}}
%\newcommand{\tKK}{\widetilde{\mathcal{K}}}
%\newcommand{\tLL}{\widetilde{\mathcal{L}}}
%\newcommand{\tMM}{\widetilde{\mathcal{M}}}
%\newcommand{\tNN}{\widetilde{\mathcal{N}}}
%\newcommand{\tOO}{\widetilde{\mathcal{O}}}
%\newcommand{\tPP}{\widetilde{\mathcal{P}}}
%\newcommand{\tQQ}{\widetilde{\mathcal{Q}}}
%\newcommand{\tRR}{\widetilde{\mathcal{R}}}
%\newcommand{\tSS}{\widetilde{\mathcal{S}}}
%\newcommand{\tTT}{\widetilde{\mathcal{T}}}
%\newcommand{\tUU}{\widetilde{\mathcal{U}}}
%\newcommand{\tVV}{\widetilde{\mathcal{V}}}
%\newcommand{\tWW}{\widetilde{\mathcal{W}}}
%\newcommand{\tXX}{\widetilde{\mathcal{X}}}
%\newcommand{\tYY}{\widetilde{\mathcal{Y}}}
%\newcommand{\tZZ}{\widetilde{\mathcal{Z}}}





% tilded
\newcommand\Wa{\wt{a}}
\newcommand\Wb{\wt{b}}
\newcommand\Wc{\wt{c}}
\newcommand\Wd{\wt{d}}
\newcommand\We{\wt{e}}
\newcommand\Wf{\wt{f}}
\newcommand\Wg{\wt{g}}
\newcommand\Wh{\wt{h}}
\newcommand\Wi{\wt{i}}
\newcommand\Wj{\wt{j}}
\newcommand\Wk{\wt{k}}
\newcommand\Wl{\wt{l}}
\newcommand\Wm{\wt{m}}
\newcommand\Wn{\wt{n}}
\newcommand\Wo{\wt{o}}
\newcommand\Wp{\wt{p}}
\newcommand\Wq{\wt{q}}
\newcommand\Wr{\wt{r}}
\newcommand\Ws{\wt{s}}
\newcommand\Wt{\wt{t}}
\newcommand\Wu{\wt{u}}
\newcommand\Wv{\wt{v}}
\newcommand\Ww{\wt{w}}
\newcommand\Wx{\wt{x}}
\newcommand\Wy{\wt{y}}
\newcommand\Wz{\wt{z}}

\newcommand\WA{\wt{A}}
\newcommand\WB{\wt{B}}
\newcommand\WC{\wt{C}}
\newcommand\WD{\wt{D}}
\newcommand\WE{\wt{E}}
\newcommand\WF{\wt{F}}
\newcommand\WG{\wt{G}}
\newcommand\WH{\wt{H}}
\newcommand\WI{\wt{I}}
\newcommand\WJ{\wt{J}}
\newcommand\WK{\wt{K}}
\newcommand\WL{\wt{L}}
\newcommand\WM{\wt{M}}
\newcommand\WN{\wt{N}}
\newcommand\WO{\wt{O}}
\newcommand\WP{\wt{P}}
\newcommand\WQ{\wt{Q}}
\newcommand\WR{\wt{R}}
\newcommand\WS{\wt{S}}
\newcommand\WT{\wt{T}}
\newcommand\WU{\wt{U}}
\newcommand\WV{\wt{V}}
\newcommand\wW{\wt{W}}
\newcommand\WX{\wt{X}}
\newcommand\WY{\wt{Y}}
\newcommand\WZ{\wt{Z}}




% Lettres grecques
\newcommand{\va}{\alpha}
\newcommand{\vb}{\beta}
\newcommand{\vg}{\gamma}
\newcommand{\vd}{\delta}
\newcommand{\ve}{\varepsilon}
\newcommand{\vz}{\zeta}
%\newcommand{\va}{\eta}
\newcommand{\vt}{\theta}
\newcommand{\vi}{\iota}
\newcommand{\vk}{\kappa}
\newcommand{\vl}{\lambda}
%\newcommand{\va}{\mu}
%\newcommand{\va}{\nu}
%\newcommand{\va}{\xi}
%\newcommand{\va}{\pi}
%\newcommand{\va}{\rho}
\newcommand{\vr}{\varrho}
\newcommand{\vs}{\sigma}
%\newcommand{\va}{\tau}
\newcommand{\vu}{\upsilon}
%\newcommand{\va}{\phi}
\newcommand{\vp}{\varphi}
%\newcommand{\va}{\chi}
%\newcommand{\va}{\psi}
\newcommand{\vo}{\omega}
\newcommand{\vD}{\Delta}
\newcommand{\vG}{\Gamma}
\newcommand{\vT}{\Theta}
\newcommand{\vL}{\Lambda}
%\newcommand{\va}{\Xi}
%\newcommand{\va}{\Pi}
\newcommand{\vS}{\Sigma}
\newcommand{\vU}{\Upsilon}
%\newcommand{\va}{\Phi}
%\newcommand{\va}{\Psi}
\newcommand{\vO}{\Omega}

==> mes-theoremes.tex <==

%%%%%%%%%%%%%%%%%%%%% LEHE %%%%%%%%%%%%%%%%%%%



\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}[section]	% Pourquoi le section ?
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{prop}[theorem]{Proposition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{open}{Question}
\newtheorem{quest}[theorem]{Question}
\newtheorem{example}{Example}
\newtheorem{rek}{Remark}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{approximation}{Approximation}
\newtheorem*{requirements}{Requirements}
\newtheorem*{issue}{Issue}
\newtheorem*{but}{But}









%%%%%%%%%%%%%%%%%%%%% BUDZ %%%%%%%%%%%%%%%%%%%



\theoremstyle{definition}

%\newtheorem{thm}{Theorem}
%\newenvironment{thmbis}[1]
%  {\renewcommand{\thethm}{\ref{#1} bis}%
%   \addtocounter{thm}{-1}%
%   \begin{thm}}
%  {\end{thm}}

%\newenvironment{preuve}{
%  \noindent \textit{Proof. }}{\hfill \(\square\) }

%\newenvironment{idproof}{
%  \noindent \textit{Sketch of proof. }}{\hfill \(\square\) }

%\newtheorem{defn}{Definition}%[section]
%\newtheorem{rem}[defn]{Remark}
%\newtheorem{rems}[defn]{Remarks}
%\newtheorem{exemple}[defn]{Example}
%\newtheorem{prop}[defn]{Proposition}
%\newtheorem{corr}[defn]{Corollary}
%\newtheorem{ex}[defn]{Example}
%\newtheorem{lem}[defn]{Lemma}
%\newtheorem{conj}[defn]{Conjecture}



